AutoAdapt: An Automated Domain Adaptation Framework for LLMs

Large language models (LLMs) excel in open domains but struggle in specialized settings with limited data and evolving knowledge. Existing domain adaptation practices rely heavily on manual trial-and-error processes, incur significant hyperparameter complexity, and are highly sensitive to data and user preferences, all under the high cost of LLM training. Moreover, the interactions and transferability of hyperparameter choices across models/domains remain poorly understood, making adaptation gains uncertain even with substantial effort. To solve these challenges, we present AutoAdapt, a novel end-to-end automated framework for efficient and reliable LLM domain adaptation. AutoAdapt leverages curated knowledge bases from literature and open-source resources to reduce expert intervention. To narrow the search space, we design a novel multi-agent debating system in which proposal and critic agents iteratively interact to align user intent and incorporate data signals and best practices into the planning process. To optimize hyperparameters under tight budgets, we propose AutoRefine, a novel LLM-based surrogate that replaces costly black-box search. Across 10 tasks, AutoAdapt achieves a 25% average relative accuracy improvement over state-of-the-art Automated Machine Learning baselines with minimal overhead.

==> arxiv/Preliminaries.tex <==
\section{Preliminaries}


\textbf{Multi-agent frameworks} have emerged as a powerful paradigm for complex decision-making tasks, enabling distributed reasoning through specialized agents that collaborate via a plethora of communication workflows. In the context of automated machine learning and domain adaptation, these frameworks allow decomposition of pipeline design into modular decisions, improving scalability and adaptability compared to monolithic approaches. 


\subsection{Bayesian Optimisation}

Bayesian optimization (BO) \cite{frazier2018tutorialbayesianoptimization} is a sequential model-based approach for optimizing expensive black-box functions. It assumes an unknown objective function \( f(\mathbf{x}) \) and models it using a probabilistic surrogate, typically a Gaussian Process (GP) \cite{beckers2021introductiongaussianprocessmodels}. The GP defines a prior over functions and updates it with observed data \( \mathcal{D}_t = \{ (\mathbf{x}_i, y_i) \}_{i=1}^t \). The posterior predictive distribution at a new point \( \mathbf{x}_* \) is:

\[\mu(\mathbf{x}_*) = k(\mathbf{x}_*, X)^\top K^{-1} \mathbf{y},\]
\[\sigma^2(\mathbf{x}_*) = k(\mathbf{x}_*, \mathbf{x}_*) - k(\mathbf{x}_*, X)^\top K^{-1} k(X, \mathbf{x}_*) \]

where \( K \) is the kernel matrix with entries \( k(\mathbf{x}_i, \mathbf{x}_j) \).

The next query point is chosen by maximizing an \textit{acquisition function} \( \alpha(\mathbf{x}) \), which balances exploration and exploitation. Common choices include:
1) \textbf{Expected Improvement (EI):}
$
\alpha_{\text{EI}}(\mathbf{x}) = \mathbb{E}[\max(0, f(\mathbf{x}) - f^+)] = (\mu(\mathbf{x}) - f^+) \Phi(z) + \sigma(\mathbf{x}) \phi(z)
$
where \( z = \frac{\mu(\mathbf{x}) - f^+}{\sigma(\mathbf{x})} \), \( f^+ \) is the best observed value, and \( \Phi, \phi \) are the CDF and PDF of the standard normal distribution.
2) \textbf{Upper Confidence Bound (UCB):}
$
\alpha_{\text{UCB}}(\mathbf{x}) = \mu(\mathbf{x}) + \kappa \sigma(\mathbf{x})
$
where \( \kappa > 0 \) controls the exploration–exploitation trade-off.


